Proving Theorems using Incremental Learning and Hindsight Experience Replay

Traditional automated theorem provers for first-order logic depend on speed-optimized search and many handcrafted heuristics that are designed to work best over a wide range of domains. Machine learning approaches in literature either depend on these traditional provers to bootstrap themselves or fall short on reaching comparable performance. In this paper, we propose a general incremental learning algorithm for training domain specific provers for first-order logic without equality, based only on a basic given-clause algorithm, but using a learned clause-scoring function. Clauses are represented as graphs and presented to transformer networks with spectral features. To address the sparsity and the initial lack of training data as well as the lack of a natural curriculum, we adapt hindsight experience replay to theorem proving, so as to be able to learn even when no proof can be found. We show that provers trained this way can match and sometimes surpass state-of-the-art traditional provers on the TPTP dataset in terms of both quantity and quality of the proofs.

==> notation_background.tex <==
\section{Notation and background}




==> related.tex <==
\section{Related Work}

This work is focused on using deep learning to train an automated theorem prover (ATP) for first-order logic (FOL) and allow it to prove theorems that were previously unproven using ATPs.  More generally it concerns solving complex search problems where a small set of related problems need to be solved.

FOL occupies the central place in mathematical logic and has been used to formulate many mathematical systems.  There has been a long history of using ATPs to prove theorems formulated in FOL \citep{boyer1986set}.  The success of these attempts has been limited because of the large search space required to solve these problems.  Many attempts have been made to improve the search space such as hand tuning weights for specific theorems \citep{quaife1992automated}, or combining sets of heuristics \citep{kovacs2013first} \citep{schulz2002brainiac}.

In addition, capable (and complex) provers such as E have seen significant improvements by incorporating machine learning techniques \citep{jakubuv2020enigma,chvalovsky2019enigma,jakubuv2019hammering}.  
By contrast, our approach is to start from a bare-bones prover and utilize machine learning to generate, via incremental learning, a prover that reaches E's performance.

In the last decade, there have been numerous attempts to leverage the power of machine learning for building strong automated theorem provers. Vampire uses machine learning. Many recent works have improved performance by augmenting existing ATPs with a deep learning module \citep{loos2017deep}. The most powerful heuristic-based provers like Vampire and E have special capability to leverage machine learning on top of synthetic heuristics. However, these methods have been handicapped by the amount of proof data available for training \cite{}. This has been limited to theorems that are provable by existing ATPs or by iterations of the learned ATP. Some recent attempts have been made to generate synthetic theorems and use them for training \citep{aygun2020learning} but the results suffered as the distribution of generated theorems is significantly different from the test theorems.

On the other hand, a number of approaches used deep reinforcement learning to solve theorems such as rlCop \citep{kaliszyk2018reinforcement} plCop \citep{zombori2020prolog} and TRAIL \cite{crouse2021deep} but have not been able to reach the performance of hand tuned provers.  
In contrast, we take inspiration from the idea of hindsight experience replay \citep{andrychowicz2017hindsight} in reinforcement learning to enrich our training dataset. Further, we build an incremental learning pipeline where training and evaluation phases are merged together instead of a separate training and evaluation phases in past work \XXX need to be reworded.

Previous methods used existing proofs to improve the search for new ones for example by constructing lemmas \citep{kaliszyk2015learning} or hints \citep{veroff1996using}.  By contrast to previous approaches which only make use of successful attempts our method, following the principle of hindsight experience replay, reframes failed proof attempts to obtain proofs of intermediary goals and uses them to generate additional positive and negative training examples.

For representation of logical formulas, many approaches have been used not limited to convolutional neural networks \citep{loos2017deep}, RNNs \citep{}, Tree LSTMs,  Graph Neural Networks \cite{glorotx2019} etc. Recently, GPT-f \citep{polu2020generative} used transformers starting from a textual representation to achieve impressive results on metamath. While transformers have been very effective in capturing long term dependencies, they lose many logical invariances present in a mathematical formulas. In contrast, we use graph representation for transformers to preserve the logical invariances. Additionally, we replace positional encoding with spectral features \citep{stachenfeld2020graph,Dwivedi2020}. 

%
\begin{itemize}
    \item
    \url{https://arxiv.org/pdf/1904.01677.pdf}, \url{http://aitp-conference.org/2019/abstract/AITP_2019_paper_19.pdf}
    
    \item
    Enigma
    \url{https://arxiv.org/pdf/1903.03182.pdf}
    According to \cite{loos2017deep}
    \begin{quote}
        The most closely related work, ENIGMA (Jakubuv and Urban, 2017), also improves clause
selection heuristics for the E theorem prover. Similar in design to n-gram approaches (but
adapted to a tree structure), ENIGMA approximates the similarity of given clauses to all
clauses that contributed to a few hundred proofs. While ENIGMA achieves fast inference using
an L2 SVM, the classifier is conjecture agnostic, meaning that it will rank each clause the same
regardless of the proof task at hand. Without taking the conjecture as input to the classifier,
success requires classifiers be tailor trained on completed proofs that are similar enough to the
conjecture, limiting generalization of this approach.
    \end{quote}
\end{itemize}


\section{Related Work: alternative take}

Machine learning has been used to improve the performance of ATPs in a number of ways.

Supervised learning was used it to identify useful lemmas that can accelerate proof search. \citep{kaliszyk2015learning}  
ENIGMA used supervised learning for clause selection in E and has shown the advantages that could be gained.  \citep{jakubuv2020enigma} \citep{jakubuv2020enigma} \citep{goertzel2020make}
On the Mizar dataset, using deep learning increased the number of theorems proven.  \citep{loos2017deep}

rlCop used reinforcement learning was used to improve the performance of tableau based methods. \citep{kaliszyk2018reinforcement}
However, given that saturation algorithms perform better in FOL the results are still below state of the art.

Some attempts have been made to use synthetic theorems generated from a given axiom set to build the training data, but these methods have been unable to show sufficient transfer to reach the performance of the best provers. \citep{aygun2020learning}

These methods share a few characteristics, they build on existing state of the art prover and they use either human data or data from heuristic prover to train the system.

One exception is TRAIL, a system that starts with bare bone saturation-based prover and applies deep reinforcement learning to learn proof guidance strategies completely from scratch.  TRAIL uses random exploration and progressively proves more problems and learns from the proofs.  It is beats existing learning based provers but does not reach the performance of E.  One possible reason is that the system is unable to learn once no more proofs are being produced.  In principle, random exploration should address this issue but given the complexity of proof search space there could be a limit to what is practically reachable by exploration.  This was the motivation for using HER as it provides learning data even from failed proof attempts.

For representation of logical formulas, many approaches have been used not limited to convolutional neural networks \citep{loos2017deep}, RNNs \citep{}, Tree LSTMs,  Graph Neural Networks \cite{glorotx2019} etc. Recently, GPT-f \citep{polu2020generative} used transformers starting from a textual representation to achieve impressive results on metamath. While transformers have been very effective in capturing long term dependencies, they lose many logical invariances present in a mathematical formulas. In contrast, we use graph representation for transformers to preserve the logical invariances. Additionally, we replace positional encoding with spectral features \citep{stachenfeld2020graph,Dwivedi2020}. 

